27 years of Spaceborne IR Astronomy: An ISO, Spitzer, WISE and NEOWISE Survey for Large-Amplitude Variability in Young Stellar Objects

Infrared observations can probe photometric variability across the full evolutionary range of young stellar objects (YSOs), from deeply embedded protostars to pre-main-sequence stars with dusty disks. We present 3-8 micron light curves extending 27 years from 1997 to 2024 obtained with three space-based IR telescopes: ISO, Spitzer and WISE. Although unevenly sampled with large gaps in coverage, these light curves show variability on time scales ranging from days to decades. We focus on the Spitzer-identified YSOs with disks and envelopes that exhibit variations of a factor of two or more in this wavelength range. We identified seven YSOs where the light curves are dominated by bursts of sustained (> 5 yr) high flux, including four that show a steep decay ending the burst and three that are ongoing as of the final observation. We find six YSOs that are undergoing declines, which may be the end of bursts that began before 1997. The most common form of variability, exhibited by 26 YSOs in our sample, show variations over time intervals of years to months but do not exhibit sustained bursts or fades. The Spitzer [3.6]-[4.5] and WISE [3.5]-[4.6] colors either increase or remain constant with increasing brightness, inconsistent with dust extinction as being the primary source of the large-amplitude variability.

==> Figure_series_completed_burst_lc.tex <==
\figsetstart
\figsetnum{5}
\figsettitle{Completed Burst Light Curves}

\figsetgrpstart
\figsetgrpnum{5.1}
\figsetgrptitle{Light Curve of J05461313-0006045}
\figsetplot{J05461313-0006045_DLC_v3.pdf}
\figsetgrpnote{The 3.6 and 4.5~$\mu$m light curves of the completed bursts. 
We label the sources of the photometry in legend. Data that may 
be affected by saturation are shown with a grey color. The legends 
also contain the Spitzer magnitudes corresponding to $\Delta m = 0$,
 and the offsets added to the (NEO)WISE magnitudes to align those 
better to the Spitzer photometry.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{5.2}
\figsetgrptitle{Light Curve of J05462569+0023416}
\figsetplot{J05462569+0023416_DLC_v3.pdf}
\figsetgrpnote{The 3.6 and 4.5~$\mu$m light curves of the completed bursts. 
We label the sources of the photometry in legend. Data that may 
be affected by saturation are shown with a grey color. The legends 
also contain the Spitzer magnitudes corresponding to $\Delta m = 0$,
 and the offsets added to the (NEO)WISE magnitudes to align those 
better to the Spitzer photometry.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{5.3}
\figsetgrptitle{Light Curve of J16271758-2405139}
\figsetplot{J16271758-2405139_DLC_v3.pdf}
\figsetgrpnote{The 3.6 and 4.5~$\mu$m light curves of the completed bursts. 
We label the sources of the photometry in legend. Data that may 
be affected by saturation are shown with a grey color. The legends 
also contain the Spitzer magnitudes corresponding to $\Delta m = 0$,
 and the offsets added to the (NEO)WISE magnitudes to align those 
better to the Spitzer photometry.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{5.4}
\figsetgrptitle{Light Curve of J16264216-2431031}
\figsetplot{J16264216-2431031_DLC_v3.pdf}
\figsetgrpnote{The 3.6 and 4.5~$\mu$m light curves of the completed bursts. 
We label the sources of the photometry in legend. Data that may 
be affected by saturation are shown with a grey color. The legends 
also contain the Spitzer magnitudes corresponding to $\Delta m = 0$,
 and the offsets added to the (NEO)WISE magnitudes to align those 
better to the Spitzer photometry.}
\figsetgrpend

\figsetend

\begin{figure}
\figurenum{5}
\plotone{J05461313-0006045_DLC_v3.pdf}
\caption{The 3.6 and 4.5~$\mu$m light curves of the completed bursts. 
We label the sources of the photometry in legend. Data that may 
be affected by saturation are shown with a grey color. The legends 
also contain the Spitzer magnitudes corresponding to $\Delta m = 0$,
 and the offsets added to the (NEO)WISE magnitudes to align those 
better to the Spitzer photometry.}
\end{figure}
